ServerlessLLM: Low-Latency Serverless Inference for Large Language Models

This paper presents ServerlessLLM, a distributed system designed to support low-latency serverless inference for Large Language Models (LLMs). By harnessing the substantial near-GPU storage and memory capacities of inference servers, ServerlessLLM achieves effective local checkpoint storage, minimizing the need for remote checkpoint downloads and ensuring efficient checkpoint loading. The design of ServerlessLLM features three core contributions: (i) \emph{fast multi-tier checkpoint loading}, featuring a new loading-optimized checkpoint format and a multi-tier loading system, fully utilizing the bandwidth of complex storage hierarchies on GPU servers; (ii) \emph{efficient live migration of LLM inference}, which enables newly initiated inferences to capitalize on local checkpoint storage while ensuring minimal user interruption; and (iii) \emph{startup-time-optimized model scheduling}, which assesses the locality statuses of checkpoints on each server and schedules the model onto servers that minimize the time to start the inference. Comprehensive evaluations, including microbenchmarks and real-world scenarios, demonstrate that ServerlessLLM dramatically outperforms state-of-the-art serverless systems, reducing latency by 10 - 200X across various LLM inference workloads.

==> format.tex <==
% \begin{table}
%   \caption{Frequency of Special Characters}
%   \label{tab:freq}
%   \begin{tabular}{ccl}
%     \toprule
%     Non-English or Math&Frequency&Comments\\
%     \midrule
%     \O & 1 in 1,000& For Swedish names\\
%     $\pi$ & 1 in 5& Common in math\\
%     \$ & 4 in 5 & Used in business\\
%     $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
%   \bottomrule
% \end{tabular}
% \end{table}

% \begin{table*}
%   \caption{Some Typical Commands}
%   \label{tab:commands}
%   \begin{tabular}{ccl}
%     \toprule
%     Command &A Number & Comments\\
%     \midrule
%     \texttt{{\char'134}author} & 100& Author \\
%     \texttt{{\char'134}table}& 300 & For tables\\
%     \texttt{{\char'134}table*}& 400& For wider tables\\
%     \bottomrule
%   \end{tabular}
% \end{table*}


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{sample-franklin}
%   \caption{1907 Franklin Model D roadster. Photograph by Harris \&
%     Ewing, Inc. [Public domain], via Wikimedia
%     Commons. (\url{https://goo.gl/VLCRBB}).}
%   \Description{A woman and a girl in white dresses sit in an open car.}
% \end{figure}

%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.

==> sec/backup_4.5_contribution_migration.tex <==
\section{Live Migration of LLM Inference}
\label{sec:migration}

% Move to Section 3.
% \sys manages checkpoints on the local storage on GPU servers, encouraging the
% serverless inference cluster to schedule a model loading request onto a GPU server with locally available checkpoints, optimizing locality. In practice, however, we observe that this locality-optimized loading decision is often complicated since
% the LLM inference has a long, unpredictable completion time, making the locality-based loading often delayed when waiting for the GPU to finish ongoing LLM inference.
% In the following, we discuss how \sys address this problem in detail.

In this section, we describe how \sys achieves live migration for LLM inference, which enables locality-driven model startup while avoiding affecting ongoing LLM inference. 

% \subsection{Problem statement}

% \subsection{Design goal}
% 1. multi-tier cache

% 2. LLM is io bounded

% (pre-load is an efficient impl)

% \subsection{Locality contention analysis}\label{sec:contention analysis}
% % 1. stateful servers
% % 2. nondeterministic inference time
% % 3. huge checkpoint
% \TODO{Queueing theory to show that (1) limited scheduling space leads to severe contention probability and (2) rebalance improves scheduling chance.}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/illustration/migration-motivation.pdf}
    % \begin{subfigure}[b]{0.7\linewidth}
    %     \includegraphics[width=\linewidth]{figs/illustration/storage_status.pdf}
    %     \caption{Storage status}
    %     \label{fig:storage-status}
    % \end{subfigure}
    % \\
    % \begin{subfigure}[b]{0.9\linewidth}
    %     \includegraphics[width=\linewidth]{figs/illustration/scheduler_illustration.pdf}
    %     \caption{Timeline of different scheduling decisions.}
    %     \label{fig:scheduler-illustration}
    % \end{subfigure}
    \caption{Analysis of different locality-driven policies}
    \label{fig:migration-illustration}
\end{figure}

% begin{table}[t!]
%   \centering
%   \caption{Feature comparison of different scheduling policies.}
%   \label{tab:feature_comparison}
%   \begin{tabular}{lccc}
%     \toprule
%     \makecell{Policy} & \makecell{Cold-start\\latency} & \makecell{Minimum impact on\\ongoing requests} & \makecell{Resource\\efficiency} \\
%     \midrule
%     Unaware (Naive) & high & \cmark & \cmark \\
%     Late-binding~\cite{} & low & \cmark & \xmark \\
%     Prediction~\cite{} & \xmark & \cmark & \cmark \\
%     Preemption~\cite{} & low & \xmark & \cmark \\
%     \sys & low & \cmark & \cmark \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\subsection{Need for Live Migration} \label{live-migration}

We consider a simple example to analyze the performance of different current approaches in supporting the checkpoint locality. In this example, we have two servers (named Server 1 and Server 2) and two models (named Model A and Model B), as illustrated in Figure~\ref{fig:migration-illustration}. Server 1 currently has Model A in DRAM and Model B in SSD and its GPU is idle, while Server 2 currently has Model B in DRAM, and its GPU is running the inference of Model A.

In Figure~\ref{fig:migration-illustration}, we analyze the performance of potential policies for starting up Model B. Our analysis is based on their impact on the latency performance of both Model A and B: 

% \begin{itemize}[leftmargin=*, itemsep=0.5mm, parsep=0.5mm]
\begin{itemize}[leftmargin=*]
    \item \emph{Availability-driven policy} chooses Server 1 currently with an available GPU, and it is agnostic to the location of Model B. As a result, the Model B's startup latency suffers while the Model A remains unaffected.
    \item \emph{Locality-driven policy} opts for the locality in choosing the server and thus launching Model B on Server 2. However, it waits for Model A to complete, making Model B suffer from a long queuing delay. Furthermore, the locality policy leaves Server 1 under-utilized, preventing all servers from being fully utilized.
    \item \emph{Preemption-driven policy} preempts Model A on Server 2 and startups Model B. It identifies that Server 1 is free and reinitiates Model A there. This policy reduces Model B's latency but results in significant downtime for Model A when it performs reloading and recomputation.
    \item \emph{Live-migration-supported locality-driven policy} prioritizes locality without disrupting Model A. It initially preloads Model A on Server 1, maintaining inference operations. When Model A is set on Server 1, its intermediate state is transferred there, continuing the inference seamlessly. Following this, Model B commences on Server 2, taking advantage of locality. This policy optimizes latency for both Models A and B. %\yao{We actually don't need to motivate that Model A has a replica on the other server. "Model B" needs to start on S2 and migrating model A to another server is possible" That's all. How to find another server and whether it's possible can be discussed later.}
\end{itemize}

As we can see, among the policies for enhancing locality, live migration stands out in effectively improving latency for both Model A and Model B.

% \mypar{(1) Serverless policy} will schedule the model onto the currently available GPU, implemented in serverless inference systems by default. With this, Model B will be loaded from disk on S1 thus experiencing a long loading latency (\ie T1) as shown in (a). Model A is not affected in this case (T2 is zero).
% % \todo{describe the situation in Figure 2} \todo{Analyzing the T1 and T2}. \andrei{checkpoint locality with respect to storage tier is not considered and additional cost $T1$ is incurred for loading model B from disk. This policy maximizes $T1$, since model is loaded from disk to memory then it is loaded to GPU memory. Model A is not interrupted, thus $T2 = 0$}

% \mypar{(2) Waiting policy} considers checkpoint locality and schedules the Model B to wait for the Model A to complete. With this, T1 involves Model A's remaining inference time, which is non-deterministic and can be up to minutes, and loading from memory. Model A is not affected in this case (T2 is zero).
% % \todo{describe the situation in Figure 2} \todo{Analyzing the T1 and T2}. \andrei{model B is loaded from memory to GPU, which is a necessary and sufficient operation to start inference, thus $T1$ is minimized. The inference process for Model A is not interrupted, thus $T2=0$. The penalty of this approach is that inference for model B is delayed in a non-deterministic way, until the inference process of Model A terminates.}

% \mypar{(3) Preemption policy} is fully optimized for locality, and it preempts Model A and startup Model B (this can be the case if the Model B has a higher priority). With this, model B is loaded from memory to GPU, mimizing $T1$, at the cost of interrupting model A inference for the duration of loading on S1 and recapturing the wasted intermediate tokens before preemption. In such a case, $T2$ is high, especially if a request is preempted multiple times.
% % \todo{describe the situation in Figure 2} \todo{Analyzing the T1 and T2}. \andrei{model B is loaded from memory to GPU, mimising $T1$, at the cost of interrupting model A inference for the duration of $T2 = T1 + \text{Model B inference time}$. $T2$ cannot be pre-determined, however assuming a priority ordering, model B completes in the minimum amount of time.}

% \mypar{(4) Live migration policy} can balance locality and the interruption on ongoing LLM inference. It schedules 
% Model B on S2 after loading and live migrating Model A to S1. In such a case, T2 is the time to finish live migration while T1 involves loading A and B. T1 can be low because both A and B's checkpoints are in memory on S1 and S2 correspondingly. Assume A and B are same in size and disk bandwidth is 10x slower, this reduces T1 to 1/5. 
% \todo{describe the situation in Figure 2} \todo{Analyzing the T1 and T2}. \andrei{model B on Server 2, minimizing $T1$ to memory-to-GPU transfer time and it schedules migration of the Model A's inference process to Server 1. The interruption time $T2$ is minimized by the locality aware server decision, since A's checkpoint is in the memory of Server 1.}

\subsection{Design Choices for Live Migration}

{\color{red}
% \subsection{}
% {\color{red}
% As shown in Figure~\ref{fig:migration-illustration}, live migration can make locality-driven inference effective since it preserves low latency in comparison with SOTA locality-driven approaches, including wait-for-locality (de-facto in cache-enabled model serving systems) and preemption-and-restart [NSDI’23].

In designing live migration for LLM inference, we first looked at the standard method: snapshotting the LLM inference and migrating it (similar to Singularity~\cite{shukla2022singularity}). Yet, this approach has notable downsides: snapshot creation and transfer are slow (taking tens of seconds~\cite{shukla2022singularity}), as they encompass the model checkpoint, runtime states (input tokens, KV cache), and extensive GPU state.

However, enabling live migration for LLM inference is challenging because: (1) LLM inference has a large [dirty](not dirty) state (i.e., KV-Cache - in the size of up to GBs) and (2) a multi-round migration (needed for avoiding interfering users) may not converge, indicating unbounded migration cost.

For (1), we propose to migrate tokens (usually 10s - 100s KB), instead of KV-Cache, since recomputing the KV-Cache based on the migrated tokens on the destination GPU is significantly faster than moving the dirty state over the network.

For (2), we propose to exploit an observation in LLM inference: recomputing the KV-Cache for current tokens on the destination GPU takes significantly less time (usually an order of magnitude shorter) than generating the same number of new tokens on the source GPU. This observation, also supported by other LLM studies [SplitWise 2023], ensures efficient convergence of multi-round migration, since the quantity of tokens generated on the source diminishes with each round.
}

\subsection{Live Migration Process}
% \yao{keep \emph{dest}(\emph{src}) consistent}. done at 2024-01-19


To address the above, we propose \emph{token-based migration}. Our proposal is based on the following insight: during inference, the model checkpoint is read-only, and the KV cache can be recalculated from tokens with low latency, usually in the range of hundreds of milliseconds. Thus, if a copy of the model checkpoint exists on another server, we can initiate the model there and then transmit all current tokens. This way, the only state transferred over the network is a list of tokens (\ie an \textit{int64} array). Even with a large batch size (64) and long sequence (\eg 100k tokens for long context LLM~\cite{claude}), the token size remains in the scale of MBs, significantly smaller than the typical sizes of the KV cache (\eg GBs) and checkpoints (\eg tens of GBs).

% We have named this approach \emph{token-based migration} for LLM inference. It involves migrating what we call \emph{intermediate tokens}, which include user input tokens and those tokens predicted so far. These tokens are already part of the LLM inference and they can be extracted at low cost.

To avoid interrupting inference while migrating tokens, we designed a two-stage process. In stage 1, the destination server (referred to as the \emph{dest} server) recalculates the KV cache using the intermediate tokens. Then, in stage 2, the \emph{dest} server receives the remaining tokens that were produced after the intermediate tokens were sent.
This two-stage process is depicted in Figure~\ref{fig:seamless migration} with its steps described below:
\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{figs/illustration/seamless-migration.pdf}
    \includegraphics[width=\linewidth]{figs/illustration/seamless-migration.pdf}
    \caption{Live migration process for LLM inference}
    \label{fig:seamless migration}
\end{figure}

\begin{enumerate}[leftmargin=*, itemsep=0.5mm, parsep=0.5mm]
    \item The model loading scheduler sends a model loading request to \emph{dest} server 
    % (denoted as migration destination) 
    to load model A into GPUs. If there is an idle instance of model A on \emph{dest} server, the scheduler skips this step.
    \item After loading, the scheduler sends a migration request carrying the address of \emph{dest} server to \emph{src} server. 
    % (denoted as migration source).
    \item Upon receiving a migrate request, \emph{src} server sets itself as ``migrating'', sends a \empty{resume} request with intermediate tokens (\ie input tokens and the output tokens produced before step 3) to \emph{dest} server if the inference is not completed. Otherwise, it immediately returns to the scheduler. 
    \item \emph{dest} server recomputes KV cache given the tokens in the resume request.
    \item Once \emph{resume} request is done, \emph{src} server stops inference, returns to the scheduler, and replies to the request router with all tokens (\ie the intermediate tokens together with the remaining tokens produced between step 3 and step 5) and a flag ``migrated''. If long-context, the collection of all tokens can be very large thus resuming takes a long time, during which many new tokens are predicted. In such a case, we can repeat the above two steps to further reduce the tokens to send between \emph{src} and \emph{dest}. \dmitrii{this multi-round migration is not clear to me}
    \item The scheduler finishes the migration, unloads model A at 
    % the migration source 
    \emph{src} server
    and starts loading model B.
    \item The request router checks the flag in the inference response. If it is ``migrated'', the request router replaces \emph{src} server with \emph{dest} server in its route table and sends all tokens to \emph{dest} server to continue inference.
\end{enumerate}

\subsection{Practical Concerns}

\mypar{Handling inference completion} 
% The self-generatin aspect 
The autoregressive nature
of LLM inference may lead to task completion at 
% the migration source 
\emph{src} server
between steps \myc{3} and \myc{5}. In such cases, 
% the migration source 
\emph{src} server
informs the request router of the inference completion as usual. Additionally, it notifies the loading scheduler, which then instructs 
% the migration destination 
\emph{dest} server
to cease resuming, terminating the migration.

\mypar{Handling server failures} \sys can manage server failures during LLM inference migration. In scenarios where 
% the migration source 
\emph{src} server
fails, if the failure happens during loading (i.e., before step \myc{2} in Figure~\ref{fig:seamless migration}), the scheduler aborts the migration and unloads the model from the destination. If the failure occurs during migration (i.e., between steps \myc{2} and \myc{3}), the scheduler directs the destination to clear any resumed KV cache and unload the model.

Additionally, in cases where 
% the migration destination 
\emph{src} server
fails, if the failure takes place during loading, the migration is canceled by the scheduler. Should the failure occur while resuming, the source notifies the scheduler of the failure and continues with the inference.

% If either server fails during the above process, the coordinator stops migration, clears the remaining states and mark the server as \emph{error}.


% \subsection{Motivation example}\label{sec:illustrative}
% % Goal: why migration?
% As shown in Fig~\ref{fig:storage-status}, scheduler needs to load model B. It has two choices, either immediately load model B from SSD on server 1, or load it from DRAM on server 2 after model A completes inference. 

% Existing serverless schedulers, without considering locality, will choose immediately available server (\ie server 1) thus suffers from long loading latency, as shown in Fig~\ref{fig:scheduler-illustration} (a).

% Prediction-based model schedulers calculate the remaining inference time of model A. However, this is no feasible for LLMs due to non-deterministic inference time. Even if we can use a statistics, such as mean latency, the decision will still be sub-optimal in most cases (Fig.~\ref{fig:migration-illustration} (b)).

% There are several methods to deal with non-deterministic task execution time. For example, late-binding, \ie the scheduler selects both server 1 and 2 to load the model checkpoints, and start inference on which ever ready first. However, this results in large IO amplification and GPU waste.
% Preemption is another choice, \ie the scheduler preempts model A on server 2 to load model B immediately. While minimising startup latency of model B, preemption results significant impact to the ongoing inference request (\ie model A).

% Migration is a promising method in such a case. For example, scheduler can migrate model A from server 2 to server 1, after which model B can be immediately started. More importantly, migration time, unlike inference, depending on IO bandwidth and model checkpoint size, is deterministic. 

% \subsection{Efficient LLM inference migration}\label{sec:llm migration}
% \begin{figure}[t]
%     \centering
%     % \includegraphics[width=\linewidth]{figs/illustration/seamless-migration.pdf}
%     \includegraphics[width=\linewidth]{figs/illustration/dist-seamless-migration.pdf}
%     \caption{Seamless migration mechanism}
%     \label{fig:seamless migration}
% \end{figure}

% Challenge 1: inefficient migration.
% While we have analysed that migration can significantly reduce the contention latency without affecting other ongoing inference, 
% However, to achieve the theoretical acceleration in LLM inference, we still need to solve two problems: 1. How to minimise migration cost? 2. How to minimise the impact on migrated models.

% Migrating a running inference model across servers is not trivial. The most common method is to create a snapshot of the container/process and restore on the destination server which means, model A's parameters have to be transferred as memory states. For machine learning models, prior work~\cite{} propose to save the GPU states (\ie \TODO{details}) and restore later which is used in existing model serving system~\cite{}. However they only save and restore models on the same server. Transferring GPU states over network can be complex and costly.

% Fortunately, we can leverage the auto-regressive generation property of LLMs to execute light-weight migration. Specifically, as aforementioned, LLMs predict the next token based on previous tokens. Therefore, to migrate an ongoing LLM inference request, the only state we need to transfer over network is a list of tokens (\ie an int64 array). Even if given long-context LLMs (\ie 100k~\cite{}) and large batch size (\ie 32), tokens are only in size of 25 MB which is significantly smaller than checkpoint size (10s GB) and KV cache (10s GB).

% However, while transferring If we naively only send current tokens, users will experience a significant latency when predicting the first token on the destination server because the model has to compute the attention to all existing tokens without KV cache.

% \subsection{Migratable inference process}\label{sec:migrable worker}

% [Problem and key idea]

% We modify the inference process by adding two interfaces to support light-weight migration of LLMs.
% \begin{itemize}[leftmargin=*]
%     \myitem{Migrate} Upon receiving a migrate request, the process copies current intermediate tokens including both input tokens (\ie user prompts) and predicted tokens. It then sends a resume request to the destination (\emph{dest}) worker indicated in migrate request. When the resume request returns, it replies to the coordinator.
%     \myitem{Resume} Upon receiving a resume request, the process calls inference library (\eg HuggingFace Transformers) to predict one token based on current tokens, during which KV cache of current tokens is calculated and stored. After the prediction, it returns.
%     \myitem{Cancel}
% \end{itemize}

% \subsection{Migration coordinator}
% In Fig.~\ref{fig:seamless migration}, we illustrate the migration process.
% \begin{enumerate}[leftmargin=*]
%     \item The coordinator sends a model loading request to \emph{dest} worker to load model A into GPUs.
%     \item After loading, the coordinator sends a migrate request to \emph{src} worker.
%     \item Upon receiving a migrate request, \emph{dest} worker set itself as ,``migrating'', sends a \empty{resume} request with intermediate tokens (\ie $t_1 - t_{100}$) to \emph{src} worker if the inference is not completed. Otherwise, it immediately returns to the coordinator. 
%     \item Upon receiving a \emph{resume} request, \emph{dest} server recomputes KV cache for intermediate tokens. The recomputed KV cache will be used to resume inference.
%     \item Once \emph{resume} request is done, \emph{src} worker stops inference, returns to the coordinator, and returns the inference request to the load balancer with current tokens and a flag ``migrated''.
%     \item The coordinator finishes the migration, unloads model A from source server, and starts loading model B.
%     \item The load balancer checks the flag in the inference response. If it is ``migrated'', the load balancer replace \emph{src} worker with \emph{dest} worker in its route table and sends current tokens to \emph{dest} worker to continue inference.
% \end{enumerate}

% \mypar{Fast-track migration}
% If there is an idle inference process of model A on \emph{dest} server, the coordinator skips step \myc{1}.

% \mypar{Long-context inference}
% If long-context, the intermediate tokens can be very large thus resuming takes long time, during which many new tokens are predicted. In such a case, we can extend by repeating step \myc{3} and \myc{4} until inference with newly created tokens is reasonably fast.

% \mypar{Failure handling}
% If either server fails during the above process, the coordinator stops migration, clears the remaining states and mark the server as \emph{error}.

% We observe that for LLM inference tasks, the generation process is iterative as shown in Fig.~\ref{fig:llm inference}. LLMs take user input tokens to predict the next token after which the predicted token is concatenated with current input tokens to get the input tokens for the next iteration.
% Theoretically, for each iteration, the output token only relies on input tokens and model parameters which are constant during inference. Therefore, to migrate a running inference task, if taking LLM inference as a white-box, we only need to move a list of input tokens (\ie int64) instead of the entire GPU states or even the process snapshot. 

% Challenge 2: huge kv cache (vllm) --> too slow if send over network; affect online user experience. 
% Even though we have analysed the feasibility of migrating a running inference task in preceding sections, the efficient implementation still remains a problem considering the potentially large inference state (\ie, KV cache).
% [LLM-based services such as ChatGPT often ] If we naively only send current tokens, users will experience a significant latency when predicting the first token on the destination server because the model has to compute the attention to all existing tokens without KV cache. However, as KV cache size increases linearly with the sequence length, transferring KV cache over network can be even worse than moving the entire checkpoint.

% We leverage a feature of inference %-- \TODO{explain the idea formally here}
% -- to design a two-stage migration mechanism to seamlessly migrate a running inference task from one server to another. 

% Fig.~\ref{fig:seamless migration} illustrates the process to migrate model A from server 2 to server 1. Upon receiving a migration request, server 1 loads model A into GPUs. After loading, server 1 requests current tokens (including input tokens and predicted tokens) from server 2, recomputes the KV cache. During 
% When required to start a new instance of model B yet local servers have no free GPU, the scheduler \myc{1} executes Alg.~\ref{alg:migration algorithm} to generate a migration plan. 
% The scheduler then \myc{2} starts a new model instance (\ie model A') on the destination server. When finished loading, \myc{3} the original model instance (\ie model A) sends current tokens (\ie input and predicted tokens) to model A' and waits for the re-computation to finish. \myc{4} model A sends the predicted tokens during the recomputation to model A' and yields occupied GPUs. Finally, model B can start loading model to GPUs. Note that when waiting for GPUs, model B's checkpoint can be pre-loaded into host memory if it's not cached yet.



==> sec/backup_4_contribution_loader_0601.tex <==
\section{Fast Multi-Tier Checkpoint Loading} \label{checkpoint-loading}

% \todo{loading optimzied store: file format, memory organization, os primitives}
% \todo{High throughput predictable loading pipeline. io contention}

In this section, we describe the design of a fast near-GPU checkpoint store, which incorporates loading-optimized checkpoints and a multi-tier loading system. 

% {
% \color{red}
% \subsection{Design Goal}
% We believe LLM checkpoint loading needs to achieve the following design goals.

% \mypar{Achieving fast loading speed} Loading latency is the main factor hinders model start up. Therefore, LLM checkpoint design must support fast loading speed.

% \mypar{Supporting multi-tier storage}
% Model checkpoints are too big and too many. So we need to store them in multi-tier storage including, ... And efficiently move when loading is needed.

% \mypar{Providing predictable loading latency}
% Predictable loading latency can assist the scheduler to decide model loading decisions based on loading speed prediction.

% \mypar{Framework agnostic}
% This design should not rely on any ML framework features, i.e., framework agnostic.


% Existing built-in checkpoint loading mechanism of ML frameworks cannot provide fast loading speed, or supporting multi-tier storage. While Safetensors can achieve relatively high loading speed, it is only optimized for loading from disk into host memory (\ie, via \texttt{mmap}). Besides, all these existing methods rely on OS to copy data, which shows unstable latency in Section~\ref{sec:evaluation_checkpoint}. Our design, described below, achieves all these design goals yet still be framework agnostic.
% }

\subsection{Loading-Optimized Checkpoints}\label{sec:model checkpoint}

\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{figs/illustration/checkpoint-manager.pdf}
    % \includegraphics[width=\linewidth]{figs/illustration/loading-tmp.pdf}
    \includegraphics[width=\linewidth]{figs/illustration/serverless-llm-loader-overview.pdf}
    \caption{Overview of fast multi-tier checkpoint loading.}
    \label{fig:checkpoint loader}
\end{figure}

\revised{
We aim to develop a checkpoint format designed for efficient loading. Our approach is driven by key insights tailored to the serverless inference environment: (i)~the loading of LLM checkpoints can be pre-scheduled and overlapped with the initialization of the inference process, thereby reducing loading latency; (ii)~since checkpoints are stored once and reloaded frequently, we can maintain them in a GPU-friendly format to facilitate direct access.
}

While designing such a checkpoint, we operate under a set of assumptions. The checkpoints have: (i)~\emph{Model execution files} which define the model architecture.
Depending on the framework, the format varies; TensorFlow typically uses protobuf files~\cite{tensorflowmodelformat}, while PyTorch employs Python scripts~\cite{torchmodelformat}. Beyond architecture, these files detail the size and shape of each tensor and include a model parallelism plan. This plan specifies the target GPU for each tensor during checkpoint loading. (ii)~\emph{Model parameter files} which stores the binary data of parameters in an LLM.
Tensors within these files can be arranged in any sequence. Runtimes such as PyTorch may also store tensor shapes as indices to compute the offset and size for each tensor.

% \dmitrii{The following text in 4.1 and 4.2 and 4.3 should be majorly simplified and shortened.
% main problem that causes high latency is the format and the serial loading latency (reminder from sec 3)
% we address the format issues by:
% (1) we separate checkpoints into GPU-sized partitions, 
% (2) we separate metadata and data, 
% (3) we streamline, and 
% (4) parallelize the loading procedure. No need to describe the algorithm, describe what it leads to 
% we address the serial latency by integrating the model loader with the scheduler
% (1) model object creation and model's data loading
% (2) Transparent memory pointer acquisition <- totally can be omitted, I cannot really understand it
% }

\revised{
\sys converts an uploaded checkpoint into a new loading-optimized format. The new format pre-partitions the checkpoint into multiple tensor binary files, each for a target GPU (Figure~\ref{fig:checkpoint loader}). Such a design permits throughput-friendly GPU-initiated sequential reads. To accelerate the GPU's performance in reading the sequential data on storage, \sys adopts Direct I/O (\eg `O\_DIRECT' in Linux) in reading those partitions, achieves higher throughput compared to the prevalent use of memory-mapped files (mmap) in current high-performance checkpoint designs.
}

% conversion has two primary goals: (i)~\emph{Support sequential chunk-based reading}: To ensure efficient sequential reading, tensors for each GPU are grouped in separate files. These files contain only the binary data of model parameters and exclude metadata such as tensor shapes, facilitating large chunk reading. (ii)~\emph{Support efficient tensor addressing}: We create 
% % index files that map 
% an index file that maps
% tensor names to a tuple of GPU id, offset, and size, facilitating the efficient restoration of tensors. The tensors are aligned with memory word sizes, facilitating direct computation of memory address and avoiding deserialization.

% \sys has an in-server model manager to load the loading-optimized checkpoints. The loading process is illustrated in Figure~\ref{fig:checkpoint loader}. 

\revised{
Additionally, the loading-optimized checkpoints are managed by an in-server model manager. This manager is capable of preloading the checkpoints into the GPU memory. Subsequently, during tensor initialization, the inference process can consult a tensor index file, which provides the tensor's offset. This offset is then utilized in conjunction with the base address of the checkpoint in the GPU memory (\ie CUDA IPC handles), to reconstruct the tensor's address within the inference process (\ie \textit{base + offset}). This design significantly minimizes the overhead associated with parsing and initializing tensor objects and circumvents the involvement of CPUs in the initialization of checkpoints. Finally, to ensure correct initialization, the inference process and the model manager conduct a synchronization.
}

\subsection{Multi-Tier Loading System}

\revised{
We have designed a multi-tier loading system that supports various storage devices, capable of achieving high throughput and predictable performance when concurrently loading checkpoints through a complex storage hierarchy.
}

The multi-tier loading system supports a range of storage devices, including local (e.g., NVMe, SATA), remote (e.g., S3 object store~\cite{aws-s3}), and in-memory (pinned memory) storage options. It employs specialized methods for efficient data retrieval and transfer across these devices.

\revised{
To maximize loading throughput, as depicted in Figure~\ref{fig:checkpoint loader}, the system achieves significant parallelism by assigning a group of dedicated threads to each I/O path connecting local storage devices. It incorporates chunk-based pinned memory management for checkpoints in the host memory, a pivotal technique for exploiting the extensive aggregated bandwidth between the GPUs and host memory. To ensure consistent loading performance, the multi-tier loading system orchestrates concurrent loading tasks through multiple queues, each corresponding to an I/O path within the storage hierarchy.
}

% To boost the checkpoint loading, we design an efficient multi-tier checkpoint loading subsystem, integrated within the model manager. This subsystem incorporates several techniques:

% \mypar{In-memory data chunk pool} We've developed an in-memory data chunk pool in \sys with three main goals:
% (i)~\emph{Utilizing parallel PCIe links}. To mitigate the bottleneck caused by a single PCIe link from storage when loading multiple models into GPUs, we employ parallel DRAM-to-GPU PCIe links to facilitate concurrent checkpoint loading across GPUs.
% (ii)~\emph{Supporting application-specific controls}. Our memory pool surpasses simple caching by providing APIs for the allocation and deallocation of memory. This enables fine-grained management of cached or evicted data chunks, based on specific requirements of the application.
% (iii)~\emph{Mitigating memory fragmentation}. We address latency and space inefficiencies caused by memory fragmentation by using fixed-size memory chunks for allocation and deallocation. 


% \mypar{Efficient data path} We've created an efficient data path in our model manager with two main strategies: 
% (i)~\emph{Exploiting direct file access}. We use direct file access (\eg `O\_DIRECT' in Linux) to avoid excessive data copying by directly reading data into user space. This method outperforms memory-mapped files (mmap), currently adopted in high-speed loaders such as Safetensors~\cite{safetensors}, which rely on system cache and lack consistent performance guarantees (critical for low latency scenarios).
% (ii)~\emph{Exploiting pinned memory}. We utilize pinned memory to eliminate redundant data copying between DRAM and GPU. This approach allows direct copying to the GPU with minimal CPU involvement, ensuring efficient use of PCIe bandwidth with a single thread.


% \mypar{Multi-stage data loading pipeline} We accommodate a multi-stage data loading pipeline to maximize throughput: 
% (i)~\emph{Support for multiple storage interfaces}. \sys offers dedicated function calls for various storage interfaces, including local storage (e.g., NVMe, SATA), remote storage (e.g., S3 object store~\cite{aws-s3}), and in-memory storage (pinned memory). It utilizes appropriate methods for efficient data access in each case.
% (ii)~\emph{Optimization for intra-stage throughput}. To leverage modern storage devices' high concurrency, \sys employs multiple threads for reading data within each storage tier, improving bandwidth utilization.
% (iii)~\emph{Efficient inter-stage coordination}. \sys uses a task queue-based pipeline for extensibility and low latency. Loading threads read storage chunks and enqueue their indices (offset and size) for the loading threads in the next tier. 
